Counting People by Estimating People Flows

Modern methods for counting people in crowded scenes rely on deep networks to estimate people densities in individual images. As such, only very few take advantage of temporal consistency in video sequences, and those that do only impose weak smoothness constraints across consecutive frames. In this paper, we advocate estimating people flows across image locations between consecutive images and inferring the people densities from these flows instead of directly regressing them. This enables us to impose much stronger constraints encoding the conservation of the number of people. As a result, it significantly boosts performance without requiring a more complex architecture. Furthermore, it allows us to exploit the correlation between people flow and optical flow to further improve the results. We also show that leveraging people conservation constraints in both a spatial and temporal manner makes it possible to train a deep crowd counting model in an active learning setting with much fewer annotations. This significantly reduces the annotation cost while still leading to similar performance to the full supervision case.

==> fig/delta.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}
\centering
\begin{tabular}{ccc}
\includegraphics[width=.33\linewidth]{images/delta/fdst.pdf}&
\includegraphics[width=.33\linewidth]{images/delta/venice.pdf}&
\includegraphics[width=.33\linewidth]{images/delta/world.pdf}
\\
\footnotesize{(a) {\bf FDST} }&
\footnotesize{(b) {\bf Venice}}&
\footnotesize{(c) {\bf WorldExpo'10} }
\end{tabular}
\vspace{-4mm}
  \caption{ {\bf Ablation study on $\delta$.}  Plot of $MAE$ w.r.t different ratio of annotations and different $\delta$ values on (a) {\bf FDST} (b) {\bf Venice} and (c) {\bf WorldExpo'10} datasets. Ablation study of \flowS{} with different $\delta$ values, as can be seen from the figure, $\delta = 0.1$ obtains the best performance.}
  \label{fig:delta}
  \end{figure*}


==> fig/gamma.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}
\centering
\begin{tabular}{ccc}
\includegraphics[width=.33\linewidth]{images/gamma/fdst.pdf}&
\includegraphics[width=.33\linewidth]{images/gamma/venice.pdf}&
\includegraphics[width=.33\linewidth]{images/gamma/world.pdf}
\\
\footnotesize{(a) {\bf FDST} }&
\footnotesize{(b) {\bf Venice}}&
\footnotesize{(c) {\bf WorldExpo'10} }
\end{tabular}
\vspace{-4mm}
  \caption{ {\bf Ablation study on $\gamma$.}  Plot of $MAE$ w.r.t different ratio of annotations and different $\gamma$ on (a) {\bf FDST} (b) {\bf Venice} and (c) {\bf WorldExpo'10} datasets. Ablation study of \flowC{} with different $\gamma$ values, as can be seen from this figure, $\gamma = 0.001$ obtains the best performance.}
  \label{fig:gamma}
  \end{figure*}


==> fig/indicator.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}
\centering
\begin{tabular}{ccc}
\includegraphics[width=.33\linewidth]{images/indicator/fdst.pdf}&
\includegraphics[width=.33\linewidth]{images/indicator/venice.pdf}&
\includegraphics[width=.33\linewidth]{images/indicator/world.pdf}
\\
\footnotesize{(a) {\bf FDST} }&
\footnotesize{(b) {\bf Venice}}&
\footnotesize{(c) {\bf WorldExpo'10} }
\end{tabular}
\vspace{-4mm}
  \caption{ {\bf Ablation study on the indicator measure to select patches to annotate.}  We plot the $MAE$ for different ratios of annotation and different indicators on (a) {\bf FDST}, (b) {\bf Venice}, and (c) {\bf WorldExpo'10}. Even though using the cycle consistency error as indicator outperforms random selection, the best results are reached when using the measure proposed in Eq.~\ref{eq:error}.}
  \label{fig:indicator}
  \end{figure*}


==> fig/neighbor.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[htbp]
\centering
 \includegraphics{images/neighbor.pdf}
\vspace{-3mm}
  \caption{ {\bf Neighborhood of each location at image plane.} For each location not at the edge of the image plane, there are nine locations reachable within a single time step, including the location itself.}
  \label{fig:neighbor}
\end{figure}



==> table/alpha_all.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
  \centering
\scalebox{0.8}{
\begin{tabular}{lcccccc}
  \toprule
  &\multicolumn{2}{c}{{\bf CrowdFlow}}&\multicolumn{2}{c}{{\bf UCSD}}&\multicolumn{2}{c}{{\bf FDST}}\\
  $\alpha$  & $MAE$ & $RMSE$  & $MAE$ & $RMSE$ & $MAE$ & $RMSE$\\
  \midrule
    0.01& 106.3& 127.2& 0.91&  1.18 & 2.41& 2.96\\
    0.1& 102.4 & 119.4 & 0.88 & \textbf{1.12}& 2.29 & 2.86\\
    1.0& \textbf{97.8} & \textbf{112.1}& \textbf{0.86} &  1.13 & \textbf{2.17} & \textbf{2.62}    \\
    10.0& 101.3 &117.7&  0.89 & 1.14& 2.32 &2.90 \\
    100.0& 109.4 & 129.2&  0.93 & 1.17 & 2.95 & 3.42\\
  \bottomrule
  \end{tabular}
}
  \caption{{\bf Ablation study of $\alpha$ on {\bf CrowdFlow}, {\bf UCSD} and {\bf FDST}.}}
  \label{tab:alpha}
\end{table}

==> table/arch.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[t]
  \centering
  \scalebox{0.78}{
    \begin{tabular}{cccc}
      \toprule
    layer & encoder & layer & decoder \\
    \midrule
     1 - 2 & 3$\times$3$\times$64 conv-1 & 1 & 3$\times$3$\times$512 conv-2\\
   & 2 $\times$ 2 max pooling & 2 & 3$\times$3$\times$512 conv-2\\
     3 - 4 & 3$\times$3$\times$128 conv-1 & 3 & 3$\times$3$\times$512 conv-2\\
    &2 $\times$ 2 max pooling  & 4  & 3$\times$3$\times$256 conv-2\\
    5 - 7 & 3$\times$3$\times$256 conv-1 & 5 & 3$\times$3$\times$128 conv-2\\
    &2 $\times$ 2 max pooling & 6 & 3$\times$3$\times$64 conv-2\\
     8 - 10 & 3$\times$3$\times$512 conv-1 & 7 & 1$\times$1$\times$10 conv-1 \\
    11 &  contextual feature~\cite{Liu19a}  & 8 & ReLU \\
    \bottomrule
    \end{tabular}
  }
  \caption{{\bf Network architecture of our model.}
  { Convolutional layers are represented as ``(kernel size) $\times$ (kernel size) $\times$ (number of filters) conv-(dilation rate)".  }}
  \label{tab:arch}
\end{table}

==> table/backbone.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
  \centering
\scalebox{0.8}{
\begin{tabular}{lcccccc}
  \toprule
  &\multicolumn{2}{c}{{\bf CrowdFlow}} &\multicolumn{2}{c}{{\bf UCSD}} &\multicolumn{2}{c}{{\bf FDST}}\\
   Model       & $MAE$ & $RMSE$ & $MAE$ & $RMSE$ & $MAE$ & $RMSE$ \\
  \midrule
  MCNN~\cite{Zhang16s}  &172.8 & 216.0 & 1.07& 1.35 &3.77 & 4.88 \\
  \mcnnC{}  & 162.7 & 199.4 & 0.98 & 1.21 & 3.42 & 4.53\\ 
  \mcnnO{}  & {\bf 154.6} & {\bf 182.1} & {\bf 0.95}&  {\bf 1.12}  &{\bf 3.29} &  {\bf 4.28}\\
  CSRNet~\cite{Li18f}  & 137.8 & 181.0 & 1.16 & 1.47 & 3.01 & 4.19\\
  \csrC{}  &124.7 & 170.2 & 1.02 & 1.33  & 2.84& 3.79\\
  \csrO{}  & {\bf 120.3} & {\bf 162.5} & {\bf 0.94} & {\bf 1.21}  & {\bf 2.62} & {\bf 3.53}\\
  \bottomrule
  \end{tabular}
}
  \caption{{\bf Ablation study of the density regressor on {\bf CrowdFlow}, {\bf UCSD} and {\bf FDST}.}}
  \label{tab:backbone}

\end{table}

==> table/beta_all.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
  \centering
\scalebox{0.8}{
\begin{tabular}{lcccccc}
  \toprule
  &\multicolumn{2}{c}{{\bf CrowdFlow}} &\multicolumn{2}{c}{{\bf UCSD}} &\multicolumn{2}{c}{{\bf FDST}}\\
  $\beta$  & $MAE$ & $RMSE$ & $MAE$ & $RMSE$ & $MAE$ & $RMSE$ \\
  \midrule
    0.000001& 97.3& 112.0 & 0.85 & 1.11 & 2.33& 2.87\\
    0.00001&  96.6& 111.8 &  0.82& 1.10 & 2.21 & 2.62 \\
    0.0001& \textbf{96.3} & \textbf{111.6}  & \textbf{0.81} & \textbf{1.07} & \textbf{2.10} & \textbf{2.46}\\
    0.001& 96.8 & 111.9 &  0.83& 1.09 & 2.16 & 2.57\\
    0.01&  97.2& 112.2 &  0.84& 1.12 & 2.42 & 2.91\\
  \bottomrule
  \end{tabular}
}
  \caption{{\bf Ablation study of $\beta$ on {\bf CrowdFlow}, {\bf UCSD} and {\bf FDST}.}}
  \label{tab:beta}

\end{table}

==> table/grid_size.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
  \centering
\scalebox{0.8}{
\begin{tabular}{lcccccc}
  \toprule
  &\multicolumn{2}{c}{{\bf CrowdFlow}} &\multicolumn{2}{c}{{\bf UCSD}} &\multicolumn{2}{c}{{\bf FDST}}\\
  Grid size  & $MAE$ & $RMSE$ & $MAE$ & $RMSE$ & $MAE$ & $RMSE$ \\
  \midrule
  1 $\times$ 1  & 115.7& 145.8  & 0.96& 1.26 & 2.36& 2.87\\
  2 $\times$ 2  & 107.9& 138.3 & 0.95& 1.21 & 2.33& 2.85\\ 
  4 $\times$ 4  & 99.3& 121.7  & 0.92& 1.16 & 2.28& 2.79\\
  8 $\times$ 8  & \textbf{97.8} & \textbf{112.1} & \textbf{0.86} & \textbf{1.13} & \textbf{2.17} & \textbf{2.62} \\
  16 $\times$ 16  &108.4 & 134.2 & 0.90 & 1.18 & 2.30 & 2.69\\
  \bottomrule
  \end{tabular}
}
  \caption{{\bf Ablation study of the grid size on {\bf CrowdFlow}, {\bf UCSD} and {\bf FDST}.}}
  \label{tab:grid}

\end{table}

==> table/ground.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
  \centering
  \scalebox{0.78}{
    \begin{tabular}{lcc}
  \toprule
  Model  & $MAE$ & $RMSE$  \\
  \midrule
  MCNN~\cite{Zhang16c} & 145.4 & 147.3  \\
  Switch-CNN~\cite{Sam17} & 52.8 & 59.5    \\
  CSRNet\cite{Li18f} & 35.8 & 50.0\\
  CAN\cite{Liu19a} & 23.5 & 38.9 \\
  ECAN\cite{Liu19a} & 20.5 & 29.9 \\
  GPC\cite{Liu19b} & 18.2 & 26.6 \\
  \oursC{} &  \textbf{15.0}  &  \textbf{19.6}   \\
  \oursGP{} &  \textbf{12.3}  &  \textbf{17.1}   \\
  \bottomrule
  \end{tabular}
  }
  \caption{ {\bf Comparative results on the Venice dataset.} }
  \label{tab:venice}
\end{table}

==> table/terminology.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[t]
  \centering
  \begin{tabular}{ |l p{70mm}|}
    \hline
    location & one pixel in the output people flow map \\
    cell & After splitting input image into $n \times n$ patches, and each of these patches is a cell \\
    tissue & a larger image patch that consists of any adjacent $a \times a $ cells, with $ a \leq n$ \\
    \hline
    \end{tabular}
  % \vspace{-3mm}
  \caption{{\bf Terminology.}}
  \label{tab:terminology}
\end{table}
